Dandelion: Certified Approximations of Elementary Functions

Elementary function operations such as sin and exp cannot in general be computed exactly on today's digital computers, and thus have to be approximated. The standard approximations in library functions typically provide only a limited set of precisions, and are too inefficient for many applications. Polynomial approximations that are customized to a limited input domain and output accuracy can provide superior performance. In fact, the Remez algorithm computes the best possible approximation for a given polynomial degree, but has so far not been formally verified. This paper presents Dandelion, an automated certificate checker for polynomial approximations of elementary functions computed with Remez-like algorithms that is fully verified in the HOL4 theorem prover. Dandelion checks whether the difference between a polynomial approximation and its target reference elementary function remains below a given error bound for all inputs in a given constraint. By extracting a verified binary with the CakeML compiler, Dandelion can validate certificates within a reasonable time, fully automating previous manually verified approximations.

==> sections/challenges.tex <==
\section{Challenges}

The overarching challenge of the project is to automate the work done in
\cite{harrison1997verifying}.
As part of the formalization of polynomial arithmetic used in the paper was
already included in HOL4, and the approach was well explained, we assumed that
most of the complexity of developing the tool and proving it correct would be in
automating the verification steps, but not in the set up.

As it turns out, John Harrison cheated at certain places that were fine for
manual proofs, but posed serious obstacles when automating them.

\subsection{Polynomial Long Division}

In the original work, polynomial long division is derived from an existentially
quantified predicate:
\begin{gather*}
  \forall p_1 p_2.\\
  \quad{}p_1\;\text{divides}\;p_2 = \exists q. \forall x. p_2 (x) = (p_1 * q) (x)
\end{gather*}

Using a HOL4 library theorem, a non-computable definition of division can be
derived.
While this definition is sufficient for manual proofs where the witness can be
provided on-the-spot, this is unsatisfactory for fully automated tools that must
be able to divide arbitrary polynomials.

A first complication was thus to define and prove correct a computable
implementation of polynomial long division in HOL4.
Our version is inspired by the Isabelle/HOL definition from
\texttt{HOL/Computational\_Algebra/Polynomial.thy} with the major difference
being that we relate the results based on semantics and not syntactically which
actually made the proof less complicated.

\subsection{Sturm Sequences}
A similar issue arises in computing sturm sequences.
Sturm sequences need the remainder from polynomial long division and thus
inherit the non-computability from polynomial division.
Similar to how polynomial division had to be reimplement, we implemented a
computable version of Sturm sequences and proved it equivalent with the
non-computable version of Harrison.
Once polynomial division was defined and proven correct properly, getting a
computable version of Sturm sequences was relatively easy.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

